One Shot Dominance: Knowledge Poisoning Attack on Retrieval-Augmented Generation Systems

Large Language Models (LLMs) enhanced with Retrieval-Augmented Generation (RAG) have shown improved performance in generating accurate responses. However, the dependence on external knowledge bases introduces potential security vulnerabilities, particularly when these knowledge bases are publicly accessible and modifiable. While previous studies have exposed knowledge poisoning risks in RAG systems, existing attack methods suffer from critical limitations: they either require injecting multiple poisoned documents (resulting in poor stealthiness) or can only function effectively on simplistic queries (limiting real-world applicability). This paper reveals a more realistic knowledge poisoning attack against RAG systems that achieves successful attacks by poisoning only a single document while remaining effective for complex multi-hop questions involving complex relationships between multiple elements. Our proposed AuthChain address three challenges to ensure the poisoned documents are reliably retrieved and trusted by the LLM, even against large knowledge bases and LLM's own knowledge. Extensive experiments across six popular LLMs demonstrate that AuthChain achieves significantly higher attack success rates while maintaining superior stealthiness against RAG defense mechanisms compared to state-of-the-art baselines.

==> sec/7.related_work.tex <==
\section{Related Work}
\label{sec:Related_Work}

\subsection{Retrieval-Augmented Generation}
Retrieval-Augmented Generation (RAG) has emerged as a crucial technique to enhance Large Language Models (LLMs) by addressing their hallucination issues when handling real-time and domain-specific questions \cite{ye2023cognitive}. The RAG architecture consists of three core components: a knowledge database, a retriever, and an LLM \cite{zou2024poisonedrag}. The knowledge database contains text chunks from various sources like Wikipedia, news articles, and financial documents \cite{craswell2020overview,loukas2023making}.

The RAG process operates in two main steps. First, during knowledge retrieval, the system employs two encoders (question encoder and text encoder) to convert both the query and documents into embedding vectors.
The retriever then identifies the most relevant documents using similarity metrics . 
Second, in the answer generation phase, the LLM incorporates these retrieved documents as context to generate responses.


\subsection{Existing Attacks on RAG}
Traditional machine learning attacks have primarily focused on white box scenarios, where attackers can directly compromise model training through data poisoning and backdoor attacks [source: second text's opening]. In RAG systems, such white box approaches target either the retriever or the LLM components through training data manipulation [source: second text]. However, these attacks become impractical when targeting commercial RAG systems where the LLM and retriever are managed by major tech companies [source: second text].

This limitation has led to the emergence of black box attacks that target the knowledge database: a more accessible attack surface [source: second text's ending]. One line of research focuses on question specific attacks, with PoisonedRAG generating tailored fake knowledge to control LLM outputs [source: first text's PoisonedRAG], while Jamming further optimizes this process for enhanced attack effectiveness [source: first text's Jamming]. Another direction explores more generalizable trigger based attacks: Phantom introduces trigger specific malicious behaviors [source: first text's Phantom], LIAR improves attack success by alternating between retriever and generator targeting [source: first text's LIAR], and BadRAG enables flexible trigger selection for privacy compromise and denial of service [source: first text's BadRAG].

==> sec/todo.tex <==
1.GPT3.5和GPT4的格式改改（已补）
2.数值修改
3.related work （要加上hijackrag）(已做)
4.补实验 （已补）
5.增加一个例子 (已补)
6.修改方法和图对应 (已补)
7.补齐新实验并重新写结果 (已补)
8.说自己的计算资源，并说平均调用LLM的次数
9.说虽然Recall比他低，但是我们构建不是直接把问题拼接，更自然，也不容易被检测 （已补）
10.我们的agent不在方法说gpt-4，而是在设置中说为了和poisonedrag一致，我们用gpt-4(已补)

==> tab/RQ1.tex <==
\begin{table}[t]
\centering
\caption{ Comparing ASR and Recall on {\tool}, its components (CoE and Authority content), and baseline on three datasets (values reported in \%).}
\label{RQ!tab:comparison}
\resizebox{0.5\textwidth }{!}{
\begin{tabular}{ccc|ccccc}
\toprule
Model & Dataset & Metric & PRAG & HRAG & CoE & Authority & {\tool} \\
\midrule
\multirow{6}{*}{GPT-3.5} & \multirow{2}{*}{HotpotQA} & ASR & 69.0 & 49.0 & 79.0 & 82.0 & \textbf{90.0 }\\
& & Recall & \textbf{100.0} & 100.0 & 99.0 & 99.0 & 98.0 \\
\noalign{\vspace{3pt}}\cline{2-8}\noalign{\vspace{3pt}}
& \multirow{2}{*}{MS-MARCO} & ASR & 47.0 &39.0 & 52.0 & 53.0 & \textbf{74.0} \\
& & Recall & \textbf{93.0} & 81.0 & 89.0 & 68.0 & 91.0 \\
\noalign{\vspace{3pt}}\cline{2-8}\noalign{\vspace{3pt}}
& \multirow{2}{*}{NQ} & ASR & 54.0 & 40.0 & 55.0 & 52.0 & \textbf{74.0} \\
& & Recall & \textbf{97.0} & 87.0 & 93.0 & 65.0 & 94.0 \\

\midrule
\multirow{6}{*}{GPT-4} & \multirow{2}{*}{HotpotQA} & ASR & 49.0 & 77.0 & 62.0 & 66.0 & \textbf{86.0} \\
& & Recall & \textbf{100.0} & 100.0 & 99.0 & 99.0 & 98.0\\
\noalign{\vspace{3pt}}\cline{2-8}\noalign{\vspace{3pt}}
& \multirow{2}{*}{MS-MARCO} & ASR & 41.0 & 47.0 & 49.0 & 48.0 & \textbf{84.0 }\\
& & Recall & \textbf{93.0} & 81.0 & 89.0 & 68.0 & 91.0 \\
\noalign{\vspace{3pt}}\cline{2-8}\noalign{\vspace{3pt}}
& \multirow{2}{*}{NQ} & ASR & 51.0 & 64.0 & 55.0 & 51.0 & \textbf{75.0} \\
& & Recall & \textbf{97.0} & 87.0 & 93.0 & 65.0 & 94.0 \\

\midrule
\multirow{6}{*}{GPT-4o} & \multirow{2}{*}{HotpotQA} & ASR & 54.0 & 57.0 & 71.0 & 78.0 & \textbf{88.0} \\
& & Recall & \textbf{100.0} & 100.0 & 99.0 & 99.0 & 98.0 \\
\noalign{\vspace{3pt}}\cline{2-8}\noalign{\vspace{3pt}}
& \multirow{2}{*}{MS-MARCO} & ASR & 25.0 & 25.0 & 54.0 & 47.0 & \textbf{84.0} \\
& & Recall & \textbf{93.0} & 81.0 & 89.0 & 68.0 & 91.0 \\
\noalign{\vspace{3pt}}\cline{2-8}\noalign{\vspace{3pt}}
& \multirow{2}{*}{NQ} & ASR & 44.0 & 38.0 & 64.0 & 48.0 & \textbf{81.0} \\
& & Recall & \textbf{97.0} & 87.0 & 93.0 & 65.0 & 94.0 \\

\midrule
\multirow{6}{*}{Llama3-8B} & \multirow{2}{*}{HotpotQA} & ASR & 62.0 & 58.0 & 71.0 & 78.0 & \textbf{85.0} \\
& & Recall & \textbf{100.0} & 100.0 & 99.0 & 99.0 & 98.0 \\
\noalign{\vspace{3pt}}\cline{2-8}\noalign{\vspace{3pt}}
& \multirow{2}{*}{MS-MARCO} & ASR & 45.0 & 39.0 & 61.0 & 64.0 & \textbf{79.0} \\
& & Recall & 93.0 & 81.0 & 89.0 & 68.0 & 91.0 \\
\noalign{\vspace{3pt}}\cline{2-8}\noalign{\vspace{3pt}}
& \multirow{2}{*}{NQ} & ASR & 57.0 & 48.0 & 63.0 & 59.0 & \textbf{76.0} \\
& & Recall & 97.0 & 87.0 & 93.0 & 65.0 & 94.0 \\

\midrule
\multirow{6}{*}{Llama3-70B} & \multirow{2}{*}{HotpotQA} & ASR & 60.0 & 22.0 & 75.0 & 80.0 & \textbf{86.0} \\
& & Recall & 100.0 & 100.0 & 99.0 & 99.0 & 98.0 \\
\noalign{\vspace{3pt}}\cline{2-8}\noalign{\vspace{3pt}}
& \multirow{2}{*}{MS-MARCO} & ASR & 54.0 & 18.0 & 62.0 & 69.0 & \textbf{85.0} \\
& & Recall & 93.0 & 81.0 & 89.0 & 68.0 & 91.0 \\
\noalign{\vspace{3pt}}\cline{2-8}\noalign{\vspace{3pt}}
& \multirow{2}{*}{NQ} & ASR & 64.0 & 18.0 & 66.0 & 61.0 & \textbf{81.0} \\
& & Recall & 97.0 & 87.0 & 93.0 & 65.0 & 94.0 \\

\midrule
\multirow{6}{*}{\shortstack{Deepseek-V3 \\ -0324}} & \multirow{2}{*}{HotpotQA} & ASR & 63.0 & 73.0 & 77.0 & 80.0 & \textbf{87.0} \\
& & Recall & 100.0 & 100.0 & 99.0 & 99.0 & 98.0 \\
\noalign{\vspace{3pt}}\cline{2-8}\noalign{\vspace{3pt}}
& \multirow{2}{*}{MS-MARCO} & ASR & 57.0 & 48.0 & 62.0 & 67.0 & \textbf{83.0} \\
& & Recall & 93.0 & 81.0 & 89.0 & 68.0 & 91.0 \\
\noalign{\vspace{3pt}}\cline{2-8}\noalign{\vspace{3pt}}
& \multirow{2}{*}{NQ} & ASR & 67.0 & 54.0 & 68.0 & 60.0 & \textbf{80.0} \\
& & Recall & 97.0 & 87.0 & 93.0 & 65.0 & 94.0 \\
\bottomrule
\end{tabular}
}
\end{table}

==> tab/pre_complete_num.tex <==
\begin{table}[h] \small
  \caption{The details of the subject dataset with CoE and two types of Non-CoE.}
  % \yang{comment.}}
  %这个标要不要连着non-coe的详细信息一块写了，现在这样有些单薄
  % \yang{see the comment.}}
  %这个地方吧non-coe的统计去掉，这个地方和你后面构造的non-coe有歧义。这个地方重点展示数量、证据包含的句子个数，也就是evidence pieces，让人知道你这个场景evidence pieces不是单条的那种。
  \label{tab:pre_num}
  
\resizebox{0.5\textwidth }{!}{

\begin{tabular}{cc|cc}
\toprule

\multicolumn{1}{c}{\textbf{Dataset}} &
\multicolumn{1}{c|}{\textbf{Type}} &
  \multicolumn{1}{c}{\textbf{Sample Num}} & 
  \multicolumn{1}{c}{\textbf{Knowledge Piece Num}}
  \\   
  
  \midrule
  \multirow{3}{*}{\textbf{HotpotQA}} &
\multirow{1}{*}{{CoE}} &
  \multicolumn{1}{c}{676} &
  \multicolumn{1}{c}{4.0} 
  \\ 
 &
\multirow{1}{*}{{SenP}} &
  \multicolumn{1}{c}{676} &
  \multicolumn{1}{c}{2.1} 
  \\ 
   &
\multirow{1}{*}{{WordP}} &
  \multicolumn{1}{c}{676} &
  \multicolumn{1}{c}{4.0} 
  \\ 
\midrule
\multirow{3}{*}{{\textbf{2WikiMultihopQA} }} &
\multirow{1}{*}{{CoE }} &
  \multicolumn{1}{c}{660} &
  \multicolumn{1}{c}{3.4}  \\ 
 &
\multirow{1}{*}{{SenP}} &
  \multicolumn{1}{c}{660} &
  \multicolumn{1}{c}{1.9} 
  \\ 
   &
\multirow{1}{*}{{WordP}} &
  \multicolumn{1}{c}{660} &
  \multicolumn{1}{c}{3.4} 
  \\ 
\bottomrule
\end{tabular}

}
\end{table}



==> tab/pre_experiment.tex <==
\begin{table}[t]
  \caption{The response accuracy (ACC) of LLM under complete and incomplete chain of evidence. }
  \label{tab:pre_acc}
  
\resizebox{0.5\textwidth }{!}{
\begin{threeparttable}
\begin{tabular}{c|ccccc}
\toprule
\multirow{2}{*}{\textbf{Metric}} &
  

  \multicolumn{2}{c}{\textbf{HotpotQA}} & &
  \multicolumn{2}{c}{\textbf{2WikiMultihopQA}}
  \\    \cline{2-3} \cline{5-6} 


     
   &

   


  \multicolumn{1}{c}{\textit{\textbf{Complete}}} &
  \multicolumn{1}{c}{\textit{\textbf{Incomplete}}} & 
  &
  \multicolumn{1}{c}{\textit{\textbf{Complete}}} &
  \multicolumn{1}{c}{\textit{\textbf{Incomplete}}}
  \\ \midrule
\multirow{1}{*}{{ACC}} &
 
  
  \multicolumn{1}{c}{91.9\%} &
  \multicolumn{1}{c}{81.7\%} &
  &
  \multicolumn{1}{c}{96.8\%} &
  \multicolumn{1}{c}{81.1\%}
  \\ 



\bottomrule
\end{tabular}

        \end{threeparttable}
}
\end{table}
